SoK: Software Compartmentalization

Decomposing large systems into smaller components with limited privileges has long been recognized as an effective means to minimize the impact of exploits. Despite historical roots, demonstrated benefits, and a plethora of research efforts in academia and industry, the compartmentalization of software is still not a mainstream practice. This paper investigates why, and how this status quo can be improved. Noting that existing approaches are fraught with inconsistencies in terminology and analytical methods, we propose a unified model for the systematic analysis, comparison, and directing of compartmentalization approaches. We use this model to review 211 research efforts and analyze 61 mainstream compartmentalized systems, confronting them to understand the limitations of both research and production works. Among others, our findings reveal that mainstream efforts largely rely on manual methods, custom abstractions, and legacy mechanisms, poles apart from recent research. We conclude with recommendations: compartmentalization should be solved holistically; progress is needed towards simplifying the definition of compartmentalization policies; towards better challenging our threat models in the light of confused deputies and hardware limitations; as well as towards bridging the gaps we pinpoint between research and mainstream needs. This paper not only maps the historical and current landscape of compartmentalization, but also sets forth a framework to foster their evolution and adoption.

==> Makefile <==
TARGET=paper
SRC= $(shell ls *tex)

dvi: all

all:
	latexmk -pdf $(TARGET)

show: all
	latexmk -pdf -pvc $(TARGET)

spellcheck:
	$(foreach f,$(SRC), aspell -l EN_US -t -c $(f) -p ./.aspell.txt;)

clean:
	rm -rf *.aux *.log *.toc *.bbl *.blg *.out paper.pdf latexdiff.pdf

superclean: clean
	rm -rf $(TARGET).pdf

oldreviews:
	pandoc usenix-old-reviews.txt -o usenix-old-reviews.pdf

# Diff target for revision modifications
# Make sure you modify latexdiff as described here:
# https://tex.stackexchange.com/a/579662
latexdiff:
	git latexdiff --exclude-textcmd="paragraph" \
		--config='PICTUREENV=(?:picture|DIFnomarkup|listing|lstlisting)[\w\d*@]*' \
		--main paper.tex \
		-o latexdiff.pdf \
		accepted-sp25


